Position Tracking using Likelihood Modeling of Channel Features with Gaussian Processes

Recent localization frameworks exploit spatial information of complex channel measurements (CMs) to estimate accurate positions even in multipath propagation scenarios. State-of-the art CM fingerprinting(FP)-based methods employ convolutional neural networks (CNN) to extract the spatial information. However, they need spatially dense data sets (associated with high acquisition and maintenance efforts) to work well -- which is rarely the case in practical applications. If such data is not available (or its quality is low), we cannot compensate the performance degradation of CNN-based FP as they do not provide statistical position estimates, which prevents a fusion with other sources of information on the observation level. We propose a novel localization framework that adapts well to sparse datasets that only contain CMs of specific areas within the environment with strong multipath propagation. Our framework compresses CMs into informative features to unravel spatial information. It then regresses Gaussian processes (GPs) for each of them, which imply statistical observation models based on distance-dependent covariance kernels. Our framework combines the trained GPs with line-of-sight ranges and a dynamics model in a particle filter. Our measurements show that our approach outperforms state-of-the-art CNN fingerprinting (0.52 m vs. 1.3 m MAE) on spatially sparse data collected in a realistic industrial indoor environment.

==> graveyard.tex <==
As discussed in section \ref{sec:trackingers}, CSLAM and error mitigation based approaches focus on the extraction of spatially deterministic signal propagation components, i.e., $\tau_{0}$ and $\epsilon_{0}$. However, other features can possibly represent diffuse components and therefore provide additional spatial information, that is also exploited in Fingerprinting approaches, especially DNN-based ones. While statistical observation models available for CSLAM and error mitigation approaches, modeling diffuse multipath is a challenging task, as the high dimensionality of channel measurements does not allow for a straightforward likelihood definition. Therefore, we propose to represent the residual information by learning spatial distributions of a limited set of informative features from recorded data. We assume that there is statistical independence between the LOS component and MPCs, both deterministic and diffuse.



\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/pipeline.pdf}
    \caption{Pipeline of the proposed tracking algorithm}
    \label{fig:pipeline}
\end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/pipeline_gpr2.pdf}
    \caption{Observation likelihood modeling pipeline}
    \label{fig:gpr}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/pipeline_aenc.pdf}
    \caption{Feature extraction pipeline. \red{feature index noch falsch!}}
    \label{fig:preproc}
\end{figure}


Therefore, we conduct a qualitative spatial analysis of the outcomes of the latent space and different architecture and training data configurations in Sec.~\ref{sec:evaluation}. Furthermore, we apply standard scaling to all latent variables, fitted to $\mathcal{F}^R$.



, which we assume as statistically independent\footnote{\textcolor{red}{need citation here}}. 


$\boldsymbol{f}_{j}^k \in \mathbb{R}^F$ of the CM magnitudes as they are intended to model the diffuse components, which originate from $S_{\nu}(\tau)$.
We train the AE on an \textit{unlabeled} set of training data $\tilde{\mathcal{R}}^R = \{ |\tilde{\boldsymbol{r}}^R_{1}|, ..., |\tilde{\boldsymbol{r}}^R_{V}|\}$, obtained in a similar environment and pre-processed according to sec. \ref{subsec:LOS}. The AE is indifferent to the anchor as it is trained to compress arbitrary CM. ENC (contracting path) is trained to compress $|\tilde{\boldsymbol{r}}^R_{v}| \in \tilde{\mathcal{R}}^R$ into the corresponding $F$ latent space variables $\boldsymbol{f}_{v}^{R} \in \mathcal{F}^R$, while the decoder path is trained to obtain an accurate reconstruction $\hat{\boldsymbol{r}}^R_{v}$ of $\tilde{\boldsymbol{r}}^R_{v}$. 


To reduce the complexity of the GP models, which is $\mathcal{O} (F^3)$ we employ sparse Gaussian regression \cite{sparse_gpr}, i.e., reducing the number of inferring points to a set of relevant latent variables. We evaluate different hyper-parameter settings, kernel functions, and numbers of inferring points in Sec.~\ref{sec:evaluation}. 


Since the likelihoods implied by our proposed framework (AE and GPR) may result in significant ambiguities, we use a particle filter to track multi-modal state distributions. We define the state vector $\boldsymbol{x}^k_p$ as containing the 2D-agent position hypothesis for particle $p \in \{1,..., P\}$. For observation modeling, we process the CMs as described in the previous sections. If LOS is classified in the LOS extraction stage (i.e. $\hat{\epsilon}_{0} = 1$), we add an additional likelihood function based on the log-likelihood $w^k_{d,j,p}$ of  $\hat{d}_{j}^k \sim \mathcal{N}(||\boldsymbol{x}^{k}_p-\boldsymbol{s}_{j}||, \sigma_d)$, similar to \eqref{eq:loglk}, where $\sigma_d$ is the sensor noise standard deviation. Since the value ranges of the GP representation of the AE latent variables is scaled, we apply additional weights $w_{d}$ and $w_{f}$ to the LOS and AE feature components, respectively. The weight $w^{k}_{p}$ for each particle are then obtained by the sums of the log-likelihoods for all anchors:

Furthermore, we investigate the use of spectral subtraction (SP-SU) \cite{KulmerDelayEst} to remove the LOS component from $\boldsymbol{r}$ to obtain $\tilde{\boldsymbol{r}}$ in the case of $\hat{\epsilon}_{0}=1$. On the other hand, if $\beta_{0}$ is below the threshold ($\hat{\epsilon}_{0}=0$), we directly forward $\boldsymbol{r}$ as $\tilde{\boldsymbol{r}}$. We then apply feature extraction to obtain the residual spatial information in $\tilde{\boldsymbol{r}}$.


\begin{figure}[tb]
    \centering%
    \includegraphics[width=\linewidth]{figures/pipeline_features1.pdf}%
    \caption{Information extraction pipeline \red{neu machen sobald klar ist was was bringt, richtig referenzieren}}%
    \label{fig:infex}%
\end{figure}%


Therefore, we first conduct a gridsearch over all subsets of the set of propagation features to obtain the most suitable combination \todo{krauscr: hier auswertungsergebnisse rein, findings}.
We compare this selection with the lowest validation losses obtained in the GPR optimazation and conclude that ...
\red{erkennt man den wert der features in den validation losses}

    \item \red{sollte warsch raus}Unlike CSLAM, we do not apply computationally demanding multipath component estimation and do not require data association and object information. Instead of focusing on deterministic MPCs originating from smooth surfaces, we also exploit spatial information originating from small scattering objects. However, we do rely on previously recorded labeled training data.
